Properties of the Top Quark

The top quark was discoverd at the CDF and D0 experiments in 1995. As the partner of the bottom quark its properties within the Standard Model are fully defined. Only the mass is a free parameter. The measurement of the top quark mass and the verification of the expected properties have been an important topic of experimental top quark physics since. In this review the recent results on top quark properties obtained by the Tevatron experiments CDF and D0 are summarised. At the advent of the LHC special emphasis is given to the basic measurement methods and the dominating systematic uncertainties.

==> Lehrverzeichnis.tex <==
\begin{enumerate}\setlength{\itemsep}{0.ex plus0.2ex}
\item Juni 2002: ~~ C++ and Object Oriented Programming, Blockkurs mit
  Übungen.
\item WS 2002/3: Übungen zu Grundlagen der Physik.
\item SS 2003: ~~~\, Programmieren in C, Vorlesung mit Übungen.
\item August 2003: C++ and Object Oriented Programming, Blockkurs mit
  Übungen.
\item WS 2003/4:  Übungen zur Teilchenphysik (Einführung in das Standardmodell).
\item SS 2004: ~~~\, Programmieren in C, Vorlesung mit Übungen.
\item WS 2005/6:  Übungen zur Physik I (Mechanik und Wärmelehre).
\item SS 2006: ~~~\, Programmieren in C, Vorlesung mit Übungen.
\item SS 2006: ~~~\,  Übungen zur Physik I (Mechanik und Wärmelehre).
\item WS 2006/7: Physik an Hadron Collidern, 2stg. Vorlesung.
\item SS 2007: ~~~\, Programmieren in C, Vorlesung mit Übungen.
\item WS 2007/8: Physik an Hadron Collidern, 2stg. Vorlesung mit Übungen.
%\item SS 2008
\item WS 2008/9: Simulation von  Hadron Kollisionen, 2stg. Vorlesung mit Übungen. 
%\item Schulvorlesung
\item SS 2002--WS 2008/9 (fortlaufend): Seminar zur Physik bei DØ und Atlas.
\item SS 2009: ~~~\, Experimentalphysik~IV: Kerne und Teilchen.\\
\hspace*{22mm}  4stg. Vorlesung mit  2stg. Übungen.
\item SS 2009: ~~~\, Seminar zum FP. Betreuung
  ausgewählter Vorträge.
\end{enumerate}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "Lebenslauf"
%%% End: 

